GPU-Accelerated Mobile Multi-view Style Transfer

An estimated 60% of smartphones sold in 2018 were equipped with multiple rear cameras, enabling a wide variety of 3D-enabled applications such as 3D Photos. The success of 3D Photo platforms (Facebook 3D Photo, Holopix, etc) depend on a steady influx of user generated content. These platforms must provide simple image manipulation tools to facilitate content creation, akin to traditional photo platforms. Artistic neural style transfer, propelled by recent advancements in GPU technology, is one such tool for enhancing traditional photos. However, naively extrapolating single-view neural style transfer to the multi-view scenario produces visually inconsistent results and is prohibitively slow on mobile devices. We present a GPU-accelerated multi-view style transfer pipeline which enforces style consistency between views with on-demand performance on mobile platforms. Our pipeline is modular and creates high quality depth and parallax effects from a stereoscopic image pair.

==> sections/future_work.tex <==
\section{Future Work}

Will probably not be a part of Extended Abstract but good to write it.

% Some future directions we can consider are creating an end-to-end neural network for this task and extrapolation to multiview videos by adding temporal constraints. 

==> sections/guided_filter.tex <==
\fboxrule=4pt%border thickness
%    \subfigimg[width=\linewidth]{A)}{example-image-a} &
\makeatletter
\setlength{\@fptop}{0pt}
\makeatother
\begin{figure}

    \begin{tabular}{c@{\hskip 0.06in}c}
    \centering
    \includegraphics[height = 1.2in]{images/guided_filter/unguided_right_styled.png}
    \includegraphics[width = 1.2in]{images/guided_filter/unguided_right_styled_cropped.jpg}&
    \end{tabular}
    \begin{tabular}{c@{\hskip 0.06in}c}
    \centering
    \fcolorbox{red}{}{\includegraphics[height = 1.2in]{images/guided_filter/right_styled.png}}
    \includegraphics[width = 1.2in]{images/guided_filter/right_styled_cropped.jpg}&
    \end{tabular}

 
    \caption{Comparison of stylized right image before (top row) and after (bottom row) applying guided filter. The highlighted regions show that applying a guided filter emphasizes the edges in the original 3D scene over edges introduced by style transfer and view synthesis.}
    \label{fig:more_results}
\end{figure}

==> sections/prior_work.tex <==
\section{Prior Work}

Will probably not be a part of Extended Abstract but good to write it.

==> tables/results_disparity_loss.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results Disparity Loss Table
\begin{table}
\begin{tabularx}{\columnwidth}{X X X X}
\hline
\multirow{2}{*}{Method} & 
\multicolumn{3}{c}{Disparity Consistency Loss} \\
& 4 Views & 8 Views & 16 Views \\
\hline 
Baseline &  & &\\
Method$_{1}$ &  & &\\
Method$_{2}$ &  & &\\
Method$_{final}$ & & &\\ 
\hline
\end{tabularx}
\caption{Disparity Consistency Loss for different methods}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/results_time_ex1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results Time Taken Table

\begin{table}
\begin{tabularx}{\columnwidth}{c c X X X}
\hline
\multicolumn{2}{c}{Method} & 
\multicolumn{3}{c}{Time taken (ms)} \\
 Name & Device & 4 Views & 8 Views & 16 Views \\
\hline 
\multirow{2}{*}{Baseline} & CPU & & & \\ 
& GPU & & & &
\multirow{2}{*}{Method_{1}} & CPU & & & \\ 
& GPU & & & &
\multirow{2}{*}{Method_{2}} & CPU & & &\\ 
& GPU & & & &
\multirow{2}{*}{Method_{final}} & CPU & & & \\ 
& GPU & & & &
\hline
\end{tabularx}
\caption{Time taken for different methods}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
